Learning Fashion Compatibility from In-the-wild Images

Complementary fashion recommendation aims at identifying items from different categories (e.g. shirt, footwear, etc.) that "go well together" as an outfit. Most existing approaches learn representation for this task using labeled outfit datasets containing manually curated compatible item combinations. In this work, we propose to learn representations for compatibility prediction from in-the-wild street fashion images through self-supervised learning by leveraging the fact that people often wear compatible outfits. Our pretext task is formulated such that the representations of different items worn by the same person are closer compared to those worn by other people. Additionally, to reduce the domain gap between in-the-wild and catalog images during inference, we introduce an adversarial loss that minimizes the difference in feature distribution between the two domains. We conduct our experiments on two popular fashion compatibility benchmarks - Polyvore and Polyvore-Disjoint outfits, and outperform existing self-supervised approaches, particularly significant in cross-dataset setting where training and testing images are from different sources.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> plots/main-plot.tex <==
\begin{figure*}[!ht]
% \centering
\noindent
\begin{minipage}{.25\textwidth}
    \centering
    \subtable[]{
        \fbox{\includegraphics[width=0.9\textwidth]{images/samples.png}}
    }
\end{minipage}%
\hfill
\begin{minipage}{.73\textwidth}
    \subtable[Without Adversarial Loss]{
        \label{adversarial-loss-tsne-normal}
        \fbox{\includegraphics[width=0.92\textwidth]{images/main-blur.png}}
    }
\end{minipage}%
\caption{}
\end{figure*}

==> plots/patches-ablation-figure.tex <==
\begin{figure}[!ht]
\centering
\noindent
\begin{minipage}{.49\columnwidth}
    \centering
    \subfloat{ % use subtable[]{} for caption
    \label{patches-ablation-compat}
        \includegraphics[width=.99\textwidth]{images/patches-ablation-compat.png}
    }
\end{minipage}% This must go next to \end{minipage}
\begin{minipage}{.49\columnwidth}
    \centering
    \subfloat{
        \label{patches-ablation-fitb}
        \includegraphics[width=.99\textwidth]{images/patches-ablation-fitb.png}
    % \resizebox{.9\linewidth}{!}{\input{plots/patches-ablation-compatibility}}
    }
\end{minipage}
\caption{Effect of varying the patch size and number of patches during inference. Increasing the number of patches significantly improves the prediction performance on the Polyvore Outfits dataset. The plots also show performance comparison with different patch sizes. \textcolor{blue}{increase size}}
\end{figure}

==> section/supplementary_old.tex <==
\appendix
\setcounter{page}{1}
This supplementary document includes additional quantitative and qualitative results that provide further insights into the results discussed in the main paper.



%@article{yolov3,
%  title={YOLOv3: An Incremental Improvement},
%  author={Redmon, Joseph and Farhadi, Ali},
%  journal = {arXiv},
%  year={2018}
%}


\section{Fashion Detector}
As discussed in section~\ref{sec: sec_setting}, our approach requires bounding boxes/segmentation masks as weak labels to extract patches from different fashion items from each person. In Table~\ref{table:main-polyvore} and Table~\ref{table:main-polyvore-disjoint} of the main paper, we provided the results with ground-truth segmentation masks from the Fashionpedia \cite{jia2020fashionpedia} dataset. With the advancements in object detection and availability of fashion datasets \cite{modanet}, it is however possible to automatically obtain these weak labels from existing models. To demonstrate this, we conduct an additional experiment with detections obtained by state-of-the-art \textsc{YOLO}-v3 detector{\footnote{Redmond and Ali, YOLOv3: An Incremental Improvement, arXiv 2018. We used the publicly available model from \href{https://github.com/simaiden/Clothing-Detection}{https://github.com/simaiden/Clothing-Detection}}} trained on the ModaNet dataset \cite{modanet}. We show a few example detections in Figure~\ref{fig:supp_inferred_bounding_boxes}. While training our model with these predicted bounding boxes, we construct positive pairs only for those images that have more than one detection. 

We compare the results on the Polyvore datasets for compatibility and fill-in-the-blank (FITB) tasks in Table~\ref{table: supp_withou_gt_boxes}. It is clear from the table that the drop in performance with detected bounding boxes is small compared to the ground-truth segmentation. Thus it is possible to train our model on large-scale real-world datasets without any supervision, and achieve competitive results to that of supervised approaches.

\begin{table}[!h]
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{1}[1]{2cm}{Our method} & \multicolumn{2}{|c|}{Polyvore Outfits} & 
\multicolumn{2}{c|}{Polyvore Disjoint} \\
\cline{2-5}
 & Compat. AUC & FITB Acc. & Compat AUC & FITB Acc. \\
\hline
GT segmentation masks & 0.85 & 55.4 & 0.82 & 54.3 \\
Predicted bounding boxes & 0.83 & 54.9 & 0.81 & 53.2 \\
\hline
\end{tabular}
\end{center}
\caption{Results on the Polyvore datasets \cite{eccv2018learning} with predicted detection boxes and ground-truth segmentation masks.}
\label{table: supp_withou_gt_boxes}
\end{table}

\clearpage

\begin{figure}
\centering
\includegraphics[scale=0.6]{images/supplementary/bounding-box-inference.png}
\caption{Bounding boxes obtained by \textsc{YOLO} trained on Modanet dataset \cite{modanet}}
\label{fig:supp_inferred_bounding_boxes}
\end{figure}

\section{Qualitative Analysis}
We first show t-sne visualization of the Polvore dataset on embeddings obtained by our proposed model in Figure~\ref{fig:supp_tsne_supplementary}. Unlike \cite{kim2020self} that learns colour and texture similarities, our embeddings trained for fashion compatibility result in compatible items that belong to different categories to cluster together tightly. Interestingly, our model is also able to capture colour and textures attributes without explicit loss functions introduced in \cite{kim2020self} to learn those attributes.

We show a few success and failure cases of our model on the compatibility and fill-in-the-blank tasks in Figure~\ref{fig:supp_compatible_noncompatible} and  Figure~\ref{fig:supp_fitb}, respectively. Notice the failure cases in Figure~\ref{fig:supp_fitb} that contain annotation ambiguities (e.g. 2nd and 3rd rows in bottom figure) where more than one candidate seem to be the right choice. It clearly shows the limitation of the existing evaluation protocol that needs be addressed.

Finally, we show the benefit of using multiple patches during inference in Figure~\ref{fig:supp_role_of_patches}. Predictions made using
% Predicting on 
multiple patches (yellow) show more robustness compared to those made using only a single patch (blue) as random selection might capture unwanted regions around edges, corners or other local patterns that are not representative of the item.

\clearpage

\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{images/tsne-polyvore-main.png}
\caption{t-sne visualization of Polyvore dataset on embeddings obtained by our model.}
\label{fig:supp_tsne_supplementary}
\end{figure}



\begin{figure*}
\centering
\fbox{\begin{subfigure}[]{}
\centering
\includegraphics[width=0.8\linewidth]{images/supplementary/compatible-new.png}
\label{fig:supp_compatible_outfits}
\end{subfigure}}%

\fbox{
\begin{subfigure}[]{}
\centering
\includegraphics[width=0.8\linewidth]{images/supplementary/non-compatible-new.png}
\label{fig:supp_noncompatible_outfits}
\end{subfigure}}
\caption{Few examples showing compatible and non-compatible outfits correctly predicted by our model}
\label{fig:supp_compatible_noncompatible}
\end{figure*}

\begin{figure}
\centering
\begin{subfigure}{}
\fbox{\includegraphics[width=0.82\linewidth]{images/supplementary/fitb-corrects.png}}
\label{fig:supp_fitb_success}
\end{subfigure}
\begin{subfigure}{}
\fbox{\includegraphics[width=0.82\linewidth]{images/supplementary/fitb-wrongs.png}}
\label{fig:supp_fitb_wrongs}
\end{subfigure}
\caption{Success (top) and failure (bottom) examples for Fill-in-the-blank task on Polyvore dataset. (top) Few examples where our model successfully predicted the right candidate where green box indicate the correct candidate selected by our model. (bottom) Few examples where our model predicted the wrong candidate where green and red boxes indicate ground-truth and predicted candidates, respectively.}
\label{fig:supp_fitb}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=0.9\linewidth]{images/supplementary/patches-new.png}
\caption{Effectiveness of multiple patches (yellow) during inference compared to single patch (blue). Green and red boxes around the candidates indicate the correct/incorrect prediction made by our model.}
\label{fig:supp_role_of_patches}
\end{figure}


%\end{comment}

==> tables/adversarial_loss.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{|c|c|c|}
\hline

\multirow{2}{1.25cm}{Method} & \multicolumn{2}{|c|}{Polyvore Outfits} \\

\cline{2-3}

 & Compat. AUC & FITB Acc. \\

\hline

 Without $L_{adv}$ & 0.82 & 54.4 \\
 With $L_{adv}$ & 0.85 & 55.4 \\

\hline

\multirow{2}{1.25cm}{Method} & \multicolumn{2}{|c|}{Polyvore Disjoint} \\

\cline{2-3}
 & Compat. AUC & FITB Acc. \\

\hline

 Without $L_{adv}$  & 0.80 & 53.6 \\
 With $L_{adv}$ & 0.82 & 54.3 \\

\hline


\end{tabular}
\end{center}
\caption{Effectiveness of the proposed adversarial training for domain adaption.}
\label{adversarial-loss-table}
\end{table}


==> tables/boxes_with_fashion_detector.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}

\hline

\multirow{1}[1]{1cm}{Method} & \multicolumn{2}{|c|}{Polyvore Outfits} & 
\multicolumn{2}{c|}{Polyvore Disjoint} \\

\cline{2-5}

 & Compat. AUC & FITB Acc. & Compat AUC & FITB Acc. \\

\hline

 Without $L_{adv}$ & 0.81 & 53.2 & 0.79 & 52.4 \\
 With $L_{adv}$ & 0.85 & 55.4 & 0.82 & 54.3 \\


\hline

\end{tabular}
\end{center}
\caption{Results on the Polyvore Outfits datasets.}
\label{table:adversarial-loss}
\end{table}



==> tables/main-both.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{|c|c|c|c|}

\hline

\multicolumn{4}{|c|}{Polyvore Outfits Dataset} \\

\hline \hline

Category & Method & Compatibility AUC & FITB Accuracy \\

\hline \hline

\multirow{4}{2.5cm}{\begin{center}Supervised\end{center}} 
 & Siamese Network \cite{eccv2018learning} & 0.85 & 54.2 \\
 & Type-Aware Network \cite{eccv2018learning} & 0.86 & 55.3 \\
 & SCE-Net \cite{iccv2019learning} & 0.91 & 61.6 \\
 & CSA-Net \cite{cvpr2020fashion} & 0.91 & 63.73 \\

\hline \hline

\multirow{11}{2.5cm}{\begin{center}Self-supervised\end{center}} 
 & Jigsaw \cite{noroozi2016unsupervised} & 0.52 & 27.9 \\
 & Rotation \cite{gidaris2018unsupervised} & 0.53 & 29.4 \\
 & AutoEncoder \cite{hinton1993autoencoders} & 0.58 & 34.0 \\
 & Colorization \cite{zhang2016colorful} & 0.63 & 34.1 \\
 & ImageNet Weights & 0.66 & 39.1 \\
 & Instance Disc. \cite{zhirong2018unsupervised} & 0.74 & 45.9 \\
 & Local Agg. \cite{zhuang2019local} & 0.74 & 46.3 \\
 & RGB Histogram \cite{kim2020self} & 0.77 & 47.2 \\
 & Texture Descriptors \cite{kim2020self} & 0.77 & 50.3 \\
 & Patch Descriptors \cite{kim2020self} & 0.83 & 54.6 \\
 & STOC \cite{kim2020self} & 0.84  & 55.8 \\

\hline \hline

\multirow{2}{2.5cm}{\centering Self-supervised (Cross domain)} 
 & STOC \cite{kim2020self} & 0.81 & 53.3 \\
%  & Proposed Method & {\bf 0.85} & {\bf 55.4} \\
& Proposed Method & {\bf 0.84} & {\bf 55.5} \\

% \vtop{\hbox{\strut Self-Supervised}\hbox{\strut (+ Cross Domain)}} & Proposed Method & 0.84 & 55.2 \\

\hline \hline

\multicolumn{4}{|c|}{Polyvore Disjoint Dataset} \\

\hline \hline

\multirow{2}[2]{2.5cm}{\centering Supervised} 
 & Siamese Network \cite{eccv2018learning} & 0.85 & 54.4 \\
 & Type-Aware Network \cite{eccv2018learning} & 0.82 & 54.1 \\
 & CSA-Net \cite{cvpr2020fashion} & 0.87 & 59.26 \\

\hline \hline

\multirow{4}[4]{2.5cm}{\begin{center}Self-Supervised\end{center}} 
 & Instance Disc. \cite{zhirong2018unsupervised} & 0.69 & 43.2 \\
 & Local Agg. \cite{zhuang2019local} & 0.73 & 46.2 \\
 & RGB Histogram \cite{kim2020self} & 0.74 & 45.7 \\
 & STOC \cite{kim2020self} & 0.81  & 54.3 \\

\hline \hline

{\centering Self-Supervised (Cross Domain)} 
%  & {\centering Proposed Method} & {\centering {\bf 0.82}} & {\centering {\bf 54.3}} \\
& {\centering Proposed Method} & {\centering {\bf 0.82}} & {\centering {\bf 54.6}} \\
 
 \hline

\end{tabular}
\end{center}
\caption{Comparison of our proposed approach on the Polyvore Outfits (top) and Polyvore Disjoint (bottom) datasets for the Compatibility Prediction and FITB tasks. Our approach achieves on-par performance when compared to a supervised siamese network and outperforms previous self-supervised approaches especially in challenging cross-domain setting.}
\label{table:main-both}
\end{table*}

==> tables/main-polyvore-disjoint.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{|c|c|c|c|}

\hline

Category & Method & Compat. AUC & FITB Acc. \\

\hline \hline

\multirow{2}[2]{2.5cm}{\centering Supervised} 
 & Siamese Network \cite{eccv2018learning} & 0.85 & 54.4 \\
 & Type-Aware Network \cite{eccv2018learning} & 0.82 & 54.1 \\
 & CSA-Net \cite{cvpr2020fashion} & 0.87 & 59.26 \\

\hline \hline

\multirow{4}[4]{2.5cm}{\begin{center}Self-Supervised\end{center}} 
 & Instance Disc. \cite{zhirong2018unsupervised} & 0.69 & 43.2 \\
 & Local Agg. \cite{zhuang2019local} & 0.73 & 46.2 \\
 & RGB Histogram \cite{kim2020self} & 0.74 & 45.7 \\
 & STOC \cite{kim2020self} & 0.81  & 54.3 \\

\hline \hline

\multirow{2}{2.5cm}{\centering Self-Supervised (Cross Domain)} 
 & \multirow{2}{2.5cm}{\centering Proposed Method} & \multirow{2}{2.cm}{\centering {\bf 0.82}} & \multirow{2}{2.5cm}{\centering {\bf 54.3}} \\
 
 & & & \\
 
\hline

\end{tabular}
\end{center}
\caption{Comparison of our proposed approach on Polyvore disjoint dataset for compatibility prediction and Fill in the blank tasks.}
\label{table:main-polyvore-disjoint}
\end{table*}



==> tables/main-polyvore.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{|c|c|c|c|}

\hline

Category & Method & Compatibility AUC & FITB Accuracy \\

\hline \hline

\multirow{4}{2.5cm}{\begin{center}Supervised\end{center}} 
 & Siamese Network \cite{eccv2018learning} & 0.85 & 54.2 \\
 & Type-Aware Network \cite{eccv2018learning} & 0.86 & 55.3 \\
 & SCE-Net \cite{iccv2019learning} & 0.91 & 61.6 \\
 & CSA-Net \cite{cvpr2020fashion} & 0.91 & 63.73 \\

\hline \hline

\multirow{11}{2.5cm}{\begin{center}Self-supervised\end{center}} 
 & Jigsaw \cite{noroozi2016unsupervised} & 0.52 & 27.9 \\
 & Rotation \cite{gidaris2018unsupervised} & 0.53 & 29.4 \\
 & AutoEncoder \cite{hinton1993autoencoders} & 0.58 & 34.0 \\
 & Colorization \cite{zhang2016colorful} & 0.63 & 34.1 \\
 & ImageNet Weights & 0.66 & 39.1 \\
 & Instance Disc. \cite{zhirong2018unsupervised} & 0.74 & 45.9 \\
 & Local Agg. \cite{zhuang2019local} & 0.74 & 46.3 \\
 & RGB Histogram \cite{kim2020self} & 0.77 & 47.2 \\
 & Texture Descriptors \cite{kim2020self} & 0.77 & 50.3 \\
 & Patch Descriptors \cite{kim2020self} & 0.83 & 54.6 \\
 & STOC \cite{kim2020self} & 0.84  & 55.8 \\

\hline \hline

\multirow{2}{2.5cm}{\centering Self-supervised (Cross domain)} 
 & STOC \cite{kim2020self} & 0.81 & 53.3 \\
 & Proposed Method & {\bf 0.85} & {\bf 55.4} \\

% \vtop{\hbox{\strut Self-Supervised}\hbox{\strut (+ Cross Domain)}} & Proposed Method & 0.84 & 55.2 \\

\hline

\end{tabular}
\end{center}
\caption{\textcolor{red}{Comparison of our proposed approach on Polyvore dataset for compatibility prediction and Fill in the blank tasks. Our approach achieves on par performance when compared to a supervised siamese network and outperforms previous self-supervised approaches, even in a cross-domain setting.}}
\label{table:main-polyvore}
\end{table*}

==> tables/predicted-boxes.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\multirow{1}[1]{2cm}{Method} & \multicolumn{2}{|c|}{Polyvore Outfits} \\
\cline{2-3}
 & Compat. AUC & FITB Acc. \\
\hline
GT Segmentation Masks & 0.85 & 55.4 \\
Predicted Bounding Boxes & 0.83 & 54.9 \\
\hline
\multirow{1}[1]{2cm}{Method} & \multicolumn{2}{|c|}{Polyvore Disjoint} \\
\cline{2-3}
 & Compat. AUC & FITB Acc. \\
\hline
GT Segmentation Masks & 0.82 & 54.3 \\
Predicted Bounding Boxes & 0.81 & 53.2 \\
\hline
\end{tabular}
\end{center}
\caption{Results on the Polyvore datasets \cite{eccv2018learning} with predicted detection boxes and ground-truth segmentation masks.}
\label{table: supp_withou_gt_boxes}
\end{table}


==> tables/predicted_boxes_content.tex <==
\centering
\begin{tabular}{|c|c|c|}
    \hline
    \multirow{2}{1.5cm}{\centering{Method}} & \multicolumn{2}{|c|}{Polyvore Outfits} \\
    \cline{2-3}
     & Compat. AUC & FITB Acc. \\
    \hline
    \multirow{2}{1.5cm}{\centering{GT Masks}} & \multirow{2}{1.5cm}{\centering{0.85}} & \multirow{2}{1.5cm}{\centering{55.4}} \\
    & & \\
    \multirow{2}{1.5cm}{\centering{Predicted BBox}} & \multirow{2}{1.5cm}{\centering{0.83}} & \multirow{2}{1.5cm}{\centering{54.9}} \\
    & & \\
    \hline
    \multirow{2}{1.5cm}{\centering{Method}} & \multicolumn{2}{|c|}{Polyvore Disjoint} \\
    \cline{2-3}
    & Compat. AUC & FITB Acc. \\
    \hline
    \multirow{2}{1.5cm}{\centering{GT Masks}} & \multirow{2}{1.5cm}{\centering{0.82}} & \multirow{2}{1.5cm}{\centering{54.3}} \\
    & & \\
    \multirow{2}{1.5cm}{\centering{Predicted BBox}} &\multirow{2}{1.5cm}{\centering{0.81}} & \multirow{2}{1.5cm}{\centering{53.2}} \\
    & & \\
    \hline
\end{tabular}

